How Knowledge Workers Think Generative AI Will (Not) Transform Their Industries

Generative AI is expected to have transformative effects in multiple knowledge industries. To better understand how knowledge workers expect generative AI may affect their industries in the future, we conducted participatory research workshops for seven different industries, with a total of 54 participants across three US cities. We describe participants' expectations of generative AI's impact, including a dominant narrative that cut across the groups' discourse: participants largely envision generative AI as a tool to perform menial work, under human review. Participants do not generally anticipate the disruptive changes to knowledge industries currently projected in common media and academic narratives. Participants do however envision generative AI may amplify four social forces currently shaping their industries: deskilling, dehumanization, disconnection, and disinformation. We describe these forces, and then we provide additional detail regarding attitudes in specific knowledge industries. We conclude with a discussion of implications and research challenges for the HCI community.

==> tables/DEPRECATED_ResearchQuestions.tex <==
%% DEPRECATED BRAINSTORM OF POSSIBLE RESEARCH QUESTIONS IN DISCUSSION

% For a summary of the research questions, see Table~\ref{table:research_questions}.
% \begin{table*}[t]
%  \centering
%  \input{tables/ResearchQuestions}
%  \caption{Key HCI Research Questions.}
%  \label{table:research_questions}
% \end{table*}

\renewcommand{\arraystretch}{1.5}
\begin{center}
\begin{tabular}{ p{1.1in} p{4.4in} }
% \textbf{Narrow view of likely \newline impacts of generative AI}
%     & Why do some knowledge workers feel they will be largely unaffected by generative AI? \\
%     & How do we raise awareness among knowledge workers of potential broad impacts of generative AI within their industries? \\
%     & What transparency artifacts are most meaningful? \\
\textbf{HITL} 
     & How do we raise awareness of the limitations of HITL? \\ 
     & How do we make better HITL systems? \\
% \textbf{Social Forces} 
%     & How will the contextual moment at which generative AI landed influence its eventual adoption and use? \\
% How might the complex interaction of generative AI with multiple trends be studied? How might these unfold in the future, and are there potential remediations? One promising direction is to facilitate representation of key stakeholders in more democratic and design justice approaches that directly intersect with technology development.
% https://www.penguinrandomhouse.com/books/653481/making-art-work-by-w-patrick-mccray/9780262044257?ref=PRHB7BD76FBDB&aid=14813&linkid=PRHB7BD76FBDB 
% https://press.uchicago.edu/ucp/books/book/chicago/A/bo195231688.html
%     & How might these effects be examined or ameliorated? \\
% How might the complex interaction of generative AI with multiple trends be studied? How might these unfold in the future, and are there potential remediations? One promising direction is to facilitate representation of key stakeholders in more democratic and design justice approaches that directly intersect with technology development.
\textbf{Deskilling}
     & What training would benefit knowledge workers, to help prepare them for likely changes? \\
% How can we make impacts of deskilling more legible to decision-makers?
     & How can we scaffold people into higher level positions, if entry-level pathways disappear? \\     
%     & How can technology guide end users and clients to human experts when needed? \\
% How can information be provided to non-experts in a way that helps them then engage meaningfully with human experts as appropriate? For example, prep them to ask better questions?
% Also, how do they not guide to humans when experts are not needed? We don't really have any solutions for this one.
\textbf{Dehumanization} 
%     & How can HCI help design and development practices evolve to center human contact when it's inherently needed? \\
     & How can we learn more about which tasks bring people meaning and joy?\\
     & How do we promote critical thinking and also prevent people from becoming lazy? \\
%     & How do we keep human-AI hybrids human ``enough''? \\
% \textbf{Disconnection} 
%     & How can HCI evolve design and development practices to center direct experience of reality? \\
%     & How can HCI help design technology that alleviates rather than promotes loneliness? \\
% \textbf{Disinformation} 
%     & How can HCI support efforts in disciplines such as trust and safety to combat new challenges with disinformation that arise from generative AI? \\
%    & How can HCI engage stakeholders in exploring the interaction of generative AI with disinformation? \\
%   & How can we educate decision-makers about how to assess evaluations of these systems, as system creators are positioning their generative AI technologies as having human-level performance?
\textbf{Guardrails} 
     & How can we design responsible AI and governance approaches that embrace complex global dynamics? \\
     & How can responsible AI assessments more fully incorporate stakeholder input? \\
% & What promising remediations for generative AI exist, beyond human review?
% \pgk{Well, the obvious solution is automated review, either review by AI systems which are trained in different ways (increasing the diversity of checks in place -- or other kinds of AI systems that aren't LLMs, and potentially have more provable safety guarantees or other guardrails }
% \pgk{Another remediation strategy is increased transparency, specifically decision audits: transparency provided through the analysis of the ``decisions'' made by a generative AI system over a longer period of time, say quarterly reports. These could be provided (with privacy guarantees and filtering) in full, or in part, for example highlighting specific errors or failure cases, flagged reports, assessments of how many decisions were contested/appealed, or reports that capture other types of errors (specific keywords used, copyright concerns, etc.)}
\end{tabular}
\end{center}

%% ADDITIONAL CONTENT FOR DEHUMANIZATION
%%
%% There is already quite a lot of chatter out there about this (and also some in our study although we don't talk about it) so probably cut:
% Beyond collaborative systems, AI interventions can be designed as educational tools that don't just write essays or solve problems, but rather directly engage in problem solving.
%%
%% LAUREN COMMENTS
%% There also seem to be pernicious things like "simulated empathy" (https://www.vice.com/en/article/n7ezkm/eating-disorder-helpline-fires-staff-transitions-to-chatbot-after-unionization) and erasing/robbing of opportunities for specialized experts to speak from their own experiences as a form of work that has relational benefits in therapy
%%
%% And how do we view "quality"? mental health is actually a great example - a therapeutic process model or call center script could be followed by AI, at least on its face, but doesn't cultivate the human-human relationship that many argue is vital to therapeutic outcomes - how do we reconcile perspectives on quality?

==> tables/DEPRECATED_industry_composites_v1.tex <==
%% ORIGINAL VERSION -- based primarily on most salient themes for each industry, rather than alignment

\begin{center}
\begin{tabular}{ p{1.15in} p{4.45in} }
 \midrule
 \textbf{Software \mbox{Development}} & \textit{Generative AI is likely to drive change across most aspects of software development, at most levels of software complexity and skill. This includes, for example, the automation of menial and boring tasks, the elimination of many entry-level roles, education for junior and senior developers, and the ability of AI to reshape low-code technology solutions and even to write production-ready code within serious software companies. Some of us worry that the time and education we invested in a lucrative career might be nullified, setting us back to where we started. Some people get into software engineering for the money, but others are motivated by their love of tinkering and solving problems, and generative AI may take over a lot of the work that brings them joy. We’re also concerned that the elimination of entry-level jobs will limit paths for new people to enter the field.} \\ 
 % change across most aspects -- widespread change
 % menial and boring tasks -- menial
 % time and education nullified -- deskilling
 % take over work that brings them joy -- dehumanization
 % elimination of entry-level jobs -- deskilling
 \midrule
 \textbf{Advertising} & \textit{Generative AI is well suited to many tasks in the advertising industry. Sadly, many jobs will go away, most immediately those related to product photography and video production. However, creative oversight will remain in the human purview, and generative AI will be an exciting brainstorming tool. A human check will be required for most generative AI work, especially to make sure it doesn’t violate brand standards or copyright. In fact, new teams may need to be created to do these checks. Our industry promotes and embraces change, but we also value human craft and often challenge the quality and value of digital content, especially when it’s automatically generated.} \\ 
 % product photography and video production -- certain jobs go away
 % tool -- tool
 % human check -- human review
 % human craft -- dehumanization
 \midrule
 \textbf{Business \mbox{Communications}} & \textit{Generative AI can do a lot of our work, and it will inevitably be adopted in our industry. Companies and employees need to adapt, learn, and ``grow with AI’’ in order to stay relevant and protect job security. The communications we produce, e.g. email notifications, often become obsolete quickly. Generative AI is a great tool to produce early drafts of these routine communications and deal efficiently with high volume production. However, generative AI will need a lot of oversight and guidance, especially to make sure it meets compliance and legal standards and is consistent with our brand voice. We can leverage our existing human approval structures to check its output.} \\
 % adapt -- medium-scale change
 % tool -- tool
 % routine work -- menial
 % oversight and guidance -- human review
 \midrule
 \textbf{Journalism} & \textit{We work in a noble profession and we are already embattled on many fronts, facing misinformation, news aggregators, vastly decreased revenue streams, and more. We are already in a weak position, with poor job security and wages, and generative AI will exacerbate ongoing job loss and the erosion of journalism as a field. We value even formulaic tasks, and generative AI may replace some of the work we most enjoy doing, like writing or photojournalism.} \\ 
 % already embattled -- social forces
 % misinformation -- disinformation
 % replace work we enjoy -- dehumanization
 \midrule
 \textbf{Law} & \textit{Generative AI can perform formulaic legal tasks like drafting or research, provided its work is reviewed by qualified attorneys, replacing entry-level positions and contributing to job loss. We’ve heard press stories about false citations, which makes us wary, even with human oversight. Generative AI is unlikely to be skilled enough to replace human professionals, and it should never make decisions, or act as lawyer, judge, or jury. However, we anticipate clients will begin to use generative AI tools to perform tasks themselves, which will often lead them to make poor decisions and end up costing them money. Regulation creates tedious legal work for which generative AI is well-suited, although its output would still need to be checked by a qualified professional. For example, generative AI might apply a complex network of privacy laws, or draft administrative paperwork associated with the legalization of marijuana.} \\
 % formulaic tasks -- menial
 % reviewed by qualified attorneys -- human review
 % replacing entry-level positions -- menial
 % unlikely to replace humans -- don't embrace the hype
 \midrule
 \textbf{Education} & \textit{Students have many ways of cheating. Generative AI is a new, somewhat more effective way of cheating that we now have to deal with. We’re in the middle of restructuring much of our curriculum for unrelated reasons like inclusion and a shift towards standards-based grading. This gives us more latitude to design new activities and experiment, so maybe there are some opportunities to work generative AI into our lessons.} \\
 % this is mostly about cheating -- don't embrace the hype
 \midrule
 \textbf{Mental Health} & \textit{We work on one of society’s most important problems: mental health is a national crisis. There is a huge shortage of qualified mental health professionals and therapy requires human-to-human connection, so we feel our jobs are extremely secure against generative AI. We are however worried about telehealth services that provide low quality service but might still undermine our job security. Generative AI may be a useful tool for simulated talk-therapy training, or as a stopgap measure when people can’t immediately access a human therapist.} \\
 % tool -- tool
 % therapy requires human-to-human connection -- would be dehumanizing if implemented
 % our jobs are extremely secure -- don't embrace the hype
 \midrule
\end{tabular}
\end{center}
